Early exercise decision in American options with dividends, stochastic volatility and jumps

Using a fast numerical technique, we investigate a large database of investor suboptimal non-exercise of short maturity American call options on dividend-paying stocks listed on the Dow Jones. The correct modelling of the discrete dividend is essential for a correct calculation of the early exercise boundary as confirmed by theoretical insights. Pricing with stochastic volatility and jumps instead of the Black-Scholes-Merton benchmark cuts by a quarter the amount lost by investors through suboptimal exercise. The remaining three quarters are largely unexplained by transaction fees and may be interpreted as an opportunity cost for the investors to monitor optimal exercise.

==> 1d-transitionPde.tex <==
% !TEX root = ../FRPpaperR1.tex

\def \Xnil{2}		% t_{l}
\def \Xone {10}		% t_{l+1}
\def \Xtwo {18}		% t_{l+2}
\def \Yone{5}		% y coord of 'x'
\def \div{.7}

\def \DistColor{red}
%\def \DistColorBack{red!50}
\def \PayoffColor{black}
%\def \PayoffColorBack{gray!50}
\def \BallSize{4.5}
%\def \BallSizeBack{1.8}



%	MAIN AXES (t, y)

	\draw[gray, very thin, ->]  (0, 0)  -- ( 21 cm, 0) node[anchor=north, black] {{\LARGE $\mathsf{time}$}};
	\draw (\Xnil,  0) node[below, yshift=-2] {{\LARGE $t_{l}$}};	 	\draw[gray, very thin] (\Xnil, 0 ) -- ++(0, 9); 	
	\draw[dashed, gray,  ->] (\Xnil, 9 ) -- +(0, 2)  node[ anchor=east, black] {{{\LARGE $\mathsf{x= S_{t_{l}}}$}}};
	
	\draw (\Xone, 0) node[below, yshift=-2] {{\LARGE $t_{l+1}$}};	 	\draw[gray, very thin] (\Xone, 0 ) -- ++(0, 9); 	
	\draw[dashed, gray,  ->] (\Xone, 9 ) -- +(0, 2)  node[ anchor=east, black] {{{\LARGE $\mathsf{y= S_{t_{l+1}}}$}} };
	
	\draw (\Xtwo, 0) node[below, yshift=-2] {{\LARGE $t_{l+2}$}};	 	\draw[gray, very thin] (\Xtwo, 0 ) -- ++(0, 9); 	
	\draw[dashed, gray,  ->] (\Xtwo, 9 ) -- +(0, 2)  node[ anchor=east, black] {{{\LARGE $\mathsf{y= S_{t_{l+2}}}$}} };

	
% 'Thin' lines getting to each y node, drawn before not to cover nodes
	
	\begin{scope}[ decoration={markings,  mark=at position 0.5 with {\arrow[>=stealth]{<}} }]
	\foreach \th in {14.036255320, 0, -14.03625532, -26.56507362, -36.86992879}{
	\draw[  \PayoffColor, loosely dashed,  postaction={decorate}]  (\Xone +.4, 7) -- ++(\th:2cm);
	}
	\foreach \th in {39.09389191, 29.35777834, 17.35403929,	3.576337396,	-17.35403929}{
	\draw[  \PayoffColor, loosely dashed,  postaction={decorate}]  (\Xone+.4, 3 ) -- ++(\th:2cm);
	}
	\foreach \th in {17.35403929,	3.576337396, -11}{
		\foreach \y in {1,9}{
			\draw[  \PayoffColor, loosely dashed,  postaction={decorate}]  (\Xone+.4, \y ) -- ++(\th:2cm);
		}
	}
	\end{scope}
	
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X0) at (\Xnil, \Yone){};	
	\node[xshift=-15] () at (X0) {{\LARGE$\mathsf{x}$}};	% 'x' label
	\node[xshift= 15] () at (\Xtwo , \Yone) {{\LARGE$\mathsf{y_{i}}$}};	% 'y_{i}' label

	\begin{scope}[ decoration={markings,  mark=at position 0.33 with {\arrow{stealth}}, mark=at position 0.66 with {\arrow{stealth}}}]

	\node[ ] (X1) at (\Xone + .2, \Yone){};
		\foreach \y in {1, 3, 5, 7, 9}{
		 \draw[ -, \PayoffColor, loosely dashed, very thick, postaction={decorate}] (\Xone , \y  ) -- (X0.east);		% Recursion steps
		 \draw[ -, \PayoffColor, loosely dashed, very thick, postaction={decorate}] (\Xtwo , \y ) -- (X1.east);		% Recursion steps
 		 \node (thisNode) at (\Xone, \y) [inner sep = \BallSize pt, ball color=\PayoffColor, circle] {};			% The nodes at the end so they are not 'covered' by lines. Black balls
	}
	\end{scope}
	
	\foreach \y in {1, 3, 5, 7, 9}{
 		 \node (thisNode) at (\Xtwo, \y) [inner sep = \BallSize pt, ball color=\PayoffColor, circle] {};				% Nodes at t_{l+2}
		 }

	\node[left, xshift=-7, fill=white] at  (\Xone , \Yone) {{\LARGE$\mathsf{y_{i}}$}};




==> 1d-transition_20150908.tex <==


\newcommand{\MyNinetyDegRot}[2]{
	\pgftransformcm{0}{1}{1}{0}{\pgfpoint{#1cm}{#2cm}}
}

\newcommand{\myGlobalTransformationBis}[2]
{
    \pgftransformcm{0}{1}{0.5}{0.7}{\pgfpoint{#1cm}{#2cm}}
}

%\newcommand{\MyGaussDist}[3]{
%	 \draw[#1,smooth,very thin] plot[domain=-#2:#2, samples=30]
%	 function {exp(-x*x/#2 )*#2 + #3};
%}

\newcommand{\MyGaussDist}[3]{
	 \draw[#1,smooth,very thin, domain=-#2:#2, samples=30] plot (\x, {exp(-\x*\x/#2 )*#2 + #3});
}

\newcommand{\MyPayoff}[2]{
	 \draw[#1, smooth,very thin, domain=-#2:#2, samples=30] plot (\x, {0.5*exp( \x/2 ) +1 });
}

\def \Xone {2}
\def \Xtwo {12}		% the "distribution" X-coordinate
\def \Xthree {8}		% the "value func." X-coordinate
\def \Yone{5}	
\def \Range{4.5}    
\def \DistGap{.5}

\def \DistColor{red}
\def \DistColorBack{red!50}
\def \PayoffColor{black}
\def \PayoffColorBack{gray!50}
\def \BallSize{4.5}
\def \BallSizeBack{3}


%	MAIN AXES (t, y)

	\draw[gray, very thin, ->]  (0, 0)  -- ( 16 cm, 0) node[anchor=north, black] {{\LARGE $\mathsf{time}$}};
	\draw (\Xone, -.2) node[below] {{\LARGE $t$}};	 	\draw[gray, very thin] (\Xone, 0 ) -- ++(0, 9); 	\draw[dashed, gray,  ->] (\Xone, 9 ) -- +(0, 2)  node[ anchor=east, black] {{{\LARGE $\mathsf{y=S_{t}}$}}};
	\node[ anchor=east, black] at (\Xthree, 11) {{{\LARGE $\mathsf{y=S_{T}}$}}};
	\draw (\Xtwo,-.2) node[below] {};					\draw[gray, very thin] (\Xtwo, 0 ) -- ++(0, 9);	\draw[gray, dashed] (\Xtwo, 9 ) -- +(0, 2);
	\draw (\Xthree,-.2) node[below] {{\LARGE $T$}};		\draw[gray, very thin] (\Xthree, 0 ) -- ++(0, 9);	\draw[gray, dashed] (\Xthree, 9 ) -- +(0, 2);
	
	
%	LABELS AND CAPTIONS

	
	\node[] () at (\Xthree, 14) {\sf{{\LARGE Value Function}}};	
	\node[ \DistColor] () at (\Xtwo + 1, 13.95)    {\sf{{\LARGE Transition Density}}};
	
	\begin{scope}[ decoration={ markings,  mark=at position 0.52 with {\arrow{>}}}]
	\node[right] (projection) at (\Xone-2, 13.5) {{\Large \textsf{\ \ projection step}}};
	\draw[>->, >=latex, \PayoffColor!50, densely dotted, postaction={ decorate}, very thick] (projection.west) -- ++ (-1.6,0);
	\node[anchor=west] (recursive) at (\Xone-2, 13) {{\Large \textsf{\ \ recursive \hspace{2pt} step}}};
	\draw[>->,  \PayoffColor, loosely dashed, postaction={ decorate}, thick] (recursive.west) -- ++ (-1.6,0);

	\end{scope}

%	VALUES AT 't'	
	\foreach \y in {1,3,5, 7, 9}{
		 \node (thisNode) at (\Xone, \y) [inner sep = \BallSize pt, ball color=\PayoffColor, circle] {};
	}


%	CONNECTING LINES
	\begin{scope}[ decoration={markings,  mark=at position 0.33 with {\arrow{>}}, mark=at position 0.66 with {\arrow{>}}}]
	
	\node[] (X0) at (\Xone, \Yone){ };	% label={[]left:{\LARGE$\mathsf{x}$}}
	\node[] at (\Xone-0.5, \Yone){{\Large $\mathsf{x}$} };
		\foreach \y in {1,3,5, 7, 9}{
		 \draw[ >->, \PayoffColor, loosely dashed,  very thick, postaction={decorate}] (\Xthree -.2, \y ) -- (X0.east);
		 \draw[ >->, \DistColor, loosely dashed,  very thick, postaction={decorate}] (\Xtwo -.2, \y ) -- (\Xtwo -1.5, \y );
		 \node (thisNode) at (\Xtwo, \y) [inner sep = \BallSize pt, ball color=\DistColor, circle] {};	% The nodes at the end so they are not 'covered' by lines
	}
	\end{scope}
	
	
%	SAMPLING OF THE DISTRIBUTION

	\begin{scope}[ decoration={markings,  mark=at position 0.33 with {\arrow{>}}, mark=at position 0.66 with {\arrow{>}}}]
	\myGlobalTransformationBis{\Xtwo}{\Yone}
	\MyGaussDist{\DistColorBack}{\Range}{\DistGap}
	\foreach \y in {-4, -2, 0,  2, 4}{
		\node (thisNode) at (\y, {exp(-\y*\y/\Range )*\Range + \DistGap } ) [inner sep = \BallSizeBack, ball color=\DistColorBack, circle] {};
		\draw[>->, >= latex, \DistColorBack, densely dotted, very thick, postaction={decorate}] (thisNode) -- (\y, 0.15);
		\draw[gray!50, very thin, ->]  (-\Yone, 0)  -- (- \Yone, 5) node[anchor=south, black] {{\Large $ \mathsf{G(x, t; y, T)}$}};
	}
	\end{scope}
	
%	SAMPLING THE PAYOFF

	\begin{scope}[ decoration={ markings,  mark=at position 0.33 with {\arrow{>}}, mark=at position 0.66 with {\arrow{>}}}]
	\myGlobalTransformationBis{\Xthree}{\Yone}
	\MyPayoff{\PayoffColorBack}{4.2} 
	\foreach \y in {-4, -2, 0,  2, 4}{
		\node (thisNode) at (\y,  {0.5*exp( \y/2 ) +1 } ) [inner sep = \BallSizeBack pt, ball color=\PayoffColorBack, circle] {};
		\node (thisOtherNode) at (\y, 0 ) [inner sep = \BallSize pt, ball color=\PayoffColor, circle] {};
		\draw[>->, >=latex, \PayoffColor!50, densely dotted, very thick, postaction={ decorate}, thick] (thisNode) -- (thisOtherNode);
		\draw[\PayoffColorBack, very thin, ->]  (-\Yone, 0)  -- (- \Yone, 5) node[anchor=south, black] {{\Large $\mathsf{V(y, T)}$}};
	}
	\end{scope}



==> Parameters_table_complete.tex <==

\begin{tabular}{|c|l||cccc||cccccccc|}
\hline
{\footnotesize Underlying } & \multirow{1}{*}{{\footnotesize BS}} & \multicolumn{4}{c||}{{\footnotesize MRT}} & \multicolumn{8}{c|}{{\footnotesize BTS}}\tabularnewline
 & {\footnotesize $\sigma_{BS}$} & {\footnotesize $\gamma$} & {\footnotesize $\sigma_{M}$} & {\footnotesize $\sigma_{\psi}$} & {\footnotesize $\mu_{\psi}$} & {\footnotesize $\gamma$} & {\footnotesize $\sigma_{\psi}$} & {\footnotesize $\mu_{\psi}$} & {\footnotesize $\omega$} & {\footnotesize $\sigma_{LT}$} & {\footnotesize $\beta$} & {\footnotesize $\rho$} & {\footnotesize $\sigma_{0}$}\tabularnewline
\hline
{\footnotesize All stocks} & {\footnotesize 0.29} & {\footnotesize 1.33} & {\footnotesize 0.22} & {\footnotesize 0.16} & {\footnotesize -0.12} & {\footnotesize 0.50} & {\footnotesize 0.18} & {\footnotesize -0.12} & {\footnotesize 0.75} & {\footnotesize 0.32} & {\footnotesize 1.52} & {\footnotesize -0.35} & {\footnotesize 0.28}\tabularnewline
{\footnotesize SP500{*}} & {\footnotesize 0.18} & {\footnotesize NA} & {\footnotesize NA} & {\footnotesize NA} & {\footnotesize NA} & {\footnotesize 0.61} & {\footnotesize 0.14} & {\footnotesize -0.09} & {\footnotesize 0.4} & {\footnotesize 0.2} & {\footnotesize 3.93} & {\footnotesize -0.52} & {\footnotesize 0.2}\tabularnewline
{\footnotesize MMM} & {\footnotesize 0.25} & {\footnotesize 1.10} & {\footnotesize 0.20} & {\footnotesize 0.11} & {\footnotesize -0.13} & {\footnotesize 0.40} & {\footnotesize 0.16} & {\footnotesize -0.12} & {\footnotesize 0.68} & {\footnotesize 0.29} & {\footnotesize 1.38} & {\footnotesize -0.44} & {\footnotesize 0.36}\tabularnewline
{\footnotesize AA} & {\footnotesize 0.38} & {\footnotesize 1.68} & {\footnotesize 0.30} & {\footnotesize 0.22} & {\footnotesize -0.14} & {\footnotesize 0.50} & {\footnotesize 0.28} & {\footnotesize -0.18} & {\footnotesize 0.88} & {\footnotesize 0.36} & {\footnotesize 1.61} & {\footnotesize -0.33} & {\footnotesize 0.34}\tabularnewline
{\footnotesize AXP} & {\footnotesize 0.34} & {\footnotesize 2.19} & {\footnotesize 0.25} & {\footnotesize 0.14} & {\footnotesize -0.11} & {\footnotesize 0.58} & {\footnotesize 0.14} & {\footnotesize -0.06} & {\footnotesize 0.78} & {\footnotesize 0.37} & {\footnotesize 1.34} & {\footnotesize -0.54} & {\footnotesize 0.33}\tabularnewline
{\footnotesize T} & {\footnotesize 0.27} & {\footnotesize 1.05} & {\footnotesize 0.21} & {\footnotesize 0.15} & {\footnotesize -0.09} & {\footnotesize 0.37} & {\footnotesize 0.16} & {\footnotesize -0.11} & {\footnotesize 0.69} & {\footnotesize 0.33} & {\footnotesize 1.48} & {\footnotesize -0.26} & {\footnotesize 0.29}\tabularnewline
{\footnotesize BAC} & {\footnotesize 0.32} & {\footnotesize 1.58} & {\footnotesize 0.24} & {\footnotesize 0.18} & {\footnotesize -0.16} & {\footnotesize 1.20} & {\footnotesize 0.18} & {\footnotesize -0.14} & {\footnotesize 0.98} & {\footnotesize 0.36} & {\footnotesize 1.60} & {\footnotesize -0.45} & {\footnotesize 0.34}\tabularnewline
{\footnotesize BA} & {\footnotesize 0.31} & {\footnotesize 1.54} & {\footnotesize 0.24} & {\footnotesize 0.15} & {\footnotesize -0.13} & {\footnotesize 0.40} & {\footnotesize 0.18} & {\footnotesize -0.12} & {\footnotesize 0.80} & {\footnotesize 0.33} & {\footnotesize 1.56} & {\footnotesize -0.37} & {\footnotesize 0.24}\tabularnewline
{\footnotesize CAT} & {\footnotesize 0.32} & {\footnotesize 1.51} & {\footnotesize 0.26} & {\footnotesize 0.13} & {\footnotesize -0.10} & {\footnotesize 0.54} & {\footnotesize 0.15} & {\footnotesize -0.06} & {\footnotesize 0.78} & {\footnotesize 0.35} & {\footnotesize 1.46} & {\footnotesize -0.37} & {\footnotesize 0.30}\tabularnewline
{\footnotesize CHV} & {\footnotesize 0.24} & {\footnotesize 1.00} & {\footnotesize 0.20} & {\footnotesize 0.12} & {\footnotesize -0.09} & {\footnotesize 0.26} & {\footnotesize 0.15} & {\footnotesize -0.10} & {\footnotesize 0.55} & {\footnotesize 0.27} & {\footnotesize 1.55} & {\footnotesize -0.26} & {\footnotesize 0.23}\tabularnewline
{\footnotesize CSCO} & {\footnotesize 0.32} & {\footnotesize 1.36} & {\footnotesize 0.25} & {\footnotesize 0.17} & {\footnotesize -0.12} & {\footnotesize 1.53} & {\footnotesize 0.08} & {\footnotesize -0.10} & {\footnotesize 1.08} & {\footnotesize 0.32} & {\footnotesize 1.88} & {\footnotesize -0.36} & {\footnotesize 0.29}\tabularnewline
{\footnotesize KO} & {\footnotesize 0.24} & {\footnotesize 1.03} & {\footnotesize 0.19} & {\footnotesize 0.13} & {\footnotesize -0.12} & {\footnotesize 0.41} & {\footnotesize 0.15} & {\footnotesize -0.11} & {\footnotesize 0.66} & {\footnotesize 0.27} & {\footnotesize 1.49} & {\footnotesize -0.34} & {\footnotesize 0.23}\tabularnewline
{\footnotesize XOM} & {\footnotesize 0.24} & {\footnotesize 0.92} & {\footnotesize 0.19} & {\footnotesize 0.15} & {\footnotesize -0.12} & {\footnotesize 0.79} & {\footnotesize 0.17} & {\footnotesize -0.12} & {\footnotesize 0.69} & {\footnotesize 0.24} & {\footnotesize 1.57} & {\footnotesize -0.38} & {\footnotesize 0.27}\tabularnewline
{\footnotesize GE} & {\footnotesize 0.27} & {\footnotesize 1.06} & {\footnotesize 0.21} & {\footnotesize 0.17} & {\footnotesize -0.14} & {\footnotesize 0.41} & {\footnotesize 0.18} & {\footnotesize -0.17} & {\footnotesize 0.83} & {\footnotesize 0.36} & {\footnotesize 1.43} & {\footnotesize -0.30} & {\footnotesize 0.34}\tabularnewline
{\footnotesize HWP} & {\footnotesize 0.37} & {\footnotesize 1.81} & {\footnotesize 0.28} & {\footnotesize 0.20} & {\footnotesize -0.13} & {\footnotesize 0.64} & {\footnotesize 0.24} & {\footnotesize -0.20} & {\footnotesize 0.98} & {\footnotesize 0.45} & {\footnotesize 1.76} & {\footnotesize -0.33} & {\footnotesize 0.31}\tabularnewline
{\footnotesize HD} & {\footnotesize 0.32} & {\footnotesize 1.45} & {\footnotesize 0.24} & {\footnotesize 0.21} & {\footnotesize -0.15} & {\footnotesize 0.43} & {\footnotesize 0.28} & {\footnotesize -0.19} & {\footnotesize 0.77} & {\footnotesize 0.38} & {\footnotesize 1.77} & {\footnotesize -0.39} & {\footnotesize 0.34}\tabularnewline
{\footnotesize INTC} & {\footnotesize 0.38} & {\footnotesize 1.82} & {\footnotesize 0.29} & {\footnotesize 0.20} & {\footnotesize -0.14} & {\footnotesize 0.38} & {\footnotesize 0.30} & {\footnotesize -0.28} & {\footnotesize 0.75} & {\footnotesize 0.36} & {\footnotesize 1.64} & {\footnotesize -0.32} & {\footnotesize 0.26}\tabularnewline
{\footnotesize IBM} & {\footnotesize 0.28} & {\footnotesize 1.81} & {\footnotesize 0.21} & {\footnotesize 0.13} & {\footnotesize -0.14} & {\footnotesize 0.51} & {\footnotesize 0.22} & {\footnotesize -0.15} & {\footnotesize 0.71} & {\footnotesize 0.29} & {\footnotesize 1.84} & {\footnotesize -0.38} & {\footnotesize 0.21}\tabularnewline
{\footnotesize JNJ} & {\footnotesize 0.22} & {\footnotesize 0.87} & {\footnotesize 0.17} & {\footnotesize 0.13} & {\footnotesize -0.10} & {\footnotesize 0.32} & {\footnotesize 0.16} & {\footnotesize -0.10} & {\footnotesize 0.67} & {\footnotesize 0.25} & {\footnotesize 1.49} & {\footnotesize -0.29} & {\footnotesize 0.24}\tabularnewline
{\footnotesize JPM} & {\footnotesize 0.33} & {\footnotesize 1.19} & {\footnotesize 0.28} & {\footnotesize 0.15} & {\footnotesize -0.10} & {\footnotesize 0.27} & {\footnotesize 0.18} & {\footnotesize -0.06} & {\footnotesize 0.64} & {\footnotesize 0.33} & {\footnotesize 1.61} & {\footnotesize -0.34} & {\footnotesize 0.26}\tabularnewline
{\footnotesize MCD} & {\footnotesize 0.25} & {\footnotesize 1.08} & {\footnotesize 0.20} & {\footnotesize 0.13} & {\footnotesize -0.11} & {\footnotesize 0.32} & {\footnotesize 0.12} & {\footnotesize -0.12} & {\footnotesize 0.65} & {\footnotesize 0.26} & {\footnotesize 1.31} & {\footnotesize -0.37} & {\footnotesize 0.25}\tabularnewline
{\footnotesize MRK} & {\footnotesize 0.27} & {\footnotesize 1.22} & {\footnotesize 0.22} & {\footnotesize 0.15} & {\footnotesize -0.11} & {\footnotesize 0.40} & {\footnotesize 0.14} & {\footnotesize -0.12} & {\footnotesize 0.80} & {\footnotesize 0.36} & {\footnotesize 1.58} & {\footnotesize -0.32} & {\footnotesize 0.24}\tabularnewline
{\footnotesize MSFT} & {\footnotesize 0.25} & {\footnotesize 1.34} & {\footnotesize 0.19} & {\footnotesize 0.17} & {\footnotesize -0.09} & {\footnotesize 0.35} & {\footnotesize 0.24} & {\footnotesize -0.13} & {\footnotesize 0.77} & {\footnotesize 0.28} & {\footnotesize 1.56} & {\footnotesize -0.22} & {\footnotesize 0.34}\tabularnewline
{\footnotesize PFE} & {\footnotesize 0.28} & {\footnotesize 1.45} & {\footnotesize 0.21} & {\footnotesize 0.17} & {\footnotesize -0.10} & {\footnotesize 0.44} & {\footnotesize 0.20} & {\footnotesize -0.13} & {\footnotesize 0.80} & {\footnotesize 0.28} & {\footnotesize 1.25} & {\footnotesize -0.20} & {\footnotesize 0.27}\tabularnewline
{\footnotesize PG} & {\footnotesize 0.21} & {\footnotesize 1.00} & {\footnotesize 0.17} & {\footnotesize 0.14} & {\footnotesize -0.11} & {\footnotesize 0.74} & {\footnotesize 0.11} & {\footnotesize -0.07} & {\footnotesize 0.57} & {\footnotesize 0.25} & {\footnotesize 1.29} & {\footnotesize -0.39} & {\footnotesize 0.22}\tabularnewline
{\footnotesize TRV} & {\footnotesize 0.29} & {\footnotesize 1.41} & {\footnotesize 0.21} & {\footnotesize 0.17} & {\footnotesize -0.08} & {\footnotesize 0.49} & {\footnotesize 0.16} & {\footnotesize -0.05} & {\footnotesize 0.82} & {\footnotesize 0.32} & {\footnotesize 1.71} & {\footnotesize -0.23} & {\footnotesize 0.27}\tabularnewline
{\footnotesize UNH} & {\footnotesize 0.33} & {\footnotesize 1.30} & {\footnotesize 0.27} & {\footnotesize 0.18} & {\footnotesize -0.16} & {\footnotesize 0.99} & {\footnotesize 0.24} & {\footnotesize -0.17} & {\footnotesize 0.93} & {\footnotesize 0.32} & {\footnotesize 1.55} & {\footnotesize -0.48} & {\footnotesize 0.28}\tabularnewline
{\footnotesize UTX} & {\footnotesize 0.27} & {\footnotesize 1.17} & {\footnotesize 0.22} & {\footnotesize 0.13} & {\footnotesize -0.11} & {\footnotesize 0.38} & {\footnotesize 0.16} & {\footnotesize -0.11} & {\footnotesize 0.66} & {\footnotesize 0.30} & {\footnotesize 1.47} & {\footnotesize -0.38} & {\footnotesize 0.26}\tabularnewline
{\footnotesize VZ} & {\footnotesize 0.28} & {\footnotesize 1.24} & {\footnotesize 0.21} & {\footnotesize 0.18} & {\footnotesize -0.11} & {\footnotesize 0.60} & {\footnotesize 0.17} & {\footnotesize -0.09} & {\footnotesize 0.74} & {\footnotesize 0.33} & {\footnotesize 1.41} & {\footnotesize -0.24} & {\footnotesize 0.33}\tabularnewline
{\footnotesize WMT} & {\footnotesize 0.26} & {\footnotesize 1.14} & {\footnotesize 0.21} & {\footnotesize 0.15} & {\footnotesize -0.09} & {\footnotesize 0.40} & {\footnotesize 0.19} & {\footnotesize -0.09} & {\footnotesize 0.71} & {\footnotesize 0.29} & {\footnotesize 1.44} & {\footnotesize -0.31} & {\footnotesize 0.26}\tabularnewline
{\footnotesize DIS} & {\footnotesize 0.29} & {\footnotesize 1.23} & {\footnotesize 0.22} & {\footnotesize 0.16} & {\footnotesize -0.09} & {\footnotesize 0.50} & {\footnotesize 0.23} & {\footnotesize -0.05} & {\footnotesize 0.74} & {\footnotesize 0.31} & {\footnotesize 1.44} & {\footnotesize -0.37} & {\footnotesize 0.26}\tabularnewline
{\footnotesize DD} & {\footnotesize 0.28} & {\footnotesize 1.25} & {\footnotesize 0.22} & {\footnotesize 0.15} & {\footnotesize -0.12} & {\footnotesize 0.37} & {\footnotesize 0.18} & {\footnotesize -0.13} & {\footnotesize 0.67} & {\footnotesize 0.28} & {\footnotesize 1.51} & {\footnotesize -0.40} & {\footnotesize 0.27}\tabularnewline
\hline
\end{tabular}



==> pde.tex <==
% !TEX root =  ../FRPpaperR1.tex

\def \Xnil{2}		% t_{l}
\def \Xone {10}		% t_{l+1}
\def \Xtwo {18}		% t_{l+2}
\def \Yone{5}		% y coord of 'x'

\def \PayoffColor{black}
\def \BallSize{4.5}

\draw[very thin,color=gray, xstep=1, ystep=1] (2, 0) grid (18 , 10.2);
	\draw[dashed, gray,  ->] (\Xnil, 9 ) -- +(0, 2)  node[ anchor=east, black] {{{\LARGE $\mathsf{y= S_{t_{ }}}$}}};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X0) at (\Xnil, \Yone){};

%	MAIN AXES (t, y)

	\draw[gray, very thin, ->]  (0, 0)  -- ( 21 cm, 0) node[anchor=north, black] {{\LARGE $\mathsf{time}$}};
	\draw (\Xnil,  0) node[below, yshift=-12] {{\LARGE $t_{l}$}};	 	\draw[gray, very thin] (\Xnil, 0 ) -- ++(0, 9); 	
%	\draw[dashed, gray,  ->] (\Xnil, 9 ) -- +(0, 2)  node[ anchor=east, black] {{{\LARGE $\mathsf{x= S_{t_{l}}}$}}};
	
	\draw (\Xone, 0) node[below, yshift=-12] {{\LARGE $t_{l+1}$}};	 	\draw[gray, very thin] (\Xone, 0 ) -- ++(0, 9); 	
%	\draw[dashed, gray,  ->] (\Xone, 9 ) -- +(0, 2)  node[ anchor=east, black] {{{\LARGE $\mathsf{y= S_{t_{l+1}}}$}} };
	
	\draw (\Xtwo, 0) node[below, yshift=-12] {{\LARGE $t_{l+2}$}};	 	\draw[gray, very thin] (\Xtwo, 0 ) -- ++(0, 9); 	
%	\draw[dashed, gray,  ->] (\Xtwo, 9 ) -- +(0, 2)  node[ anchor=east, black] {{{\LARGE $\mathsf{y= S_{t_{l+2}}}$}} };
	
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X0) at (5, \Yone){};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X1) at (6, \Yone+1){};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X2) at (6, \Yone){};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X3) at (6, \Yone-1){};
	\draw[dashed, gray,  ->] (X0) -- (X1)  node[ anchor=east, black] {};
	\draw[dashed, gray,  ->] (X0) -- (X2)  node[ anchor=east, black] {};
	\draw[dashed, gray,  ->] (X0) -- (X3)  node[ anchor=east, black] {};
	
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X4) at (10, 7){};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X5) at (11, 6){};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X6) at (11, 7){};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X7) at (11, 8){};
	\draw[dashed, gray,  ->] (X4) -- (X5)  node[ anchor=east, black] {};
	\draw[dashed, gray,  ->] (X4) -- (X6)  node[ anchor=east, black] {};
	\draw[dashed, gray,  ->] (X4) -- (X7)  node[ anchor=east, black] {};	
	
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X8) at (17, 9){};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X9) at (18, 10){};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X10) at (18, 9){};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X11) at (18, 8){};
	\draw[dashed, gray,  ->] (X8) -- (X10)  node[ anchor=east, black] {};
	\draw[dashed, gray,  ->] (X8) -- (X9)  node[ anchor=east, black] {};
	\draw[dashed, gray,  ->] (X8) -- (X11)  node[ anchor=east, black] {};	
	
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X12) at (16, 8){};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X13) at (17, 7){};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X14) at (17, 9){};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X15) at (17, 8){};
	\draw[dashed, gray,  ->] (X12) -- (X13)  node[ anchor=east, black] {};
	\draw[dashed, gray,  ->] (X12) -- (X14)  node[ anchor=east, black] {};
	\draw[dashed, gray,  ->] (X12) -- (X15)  node[ anchor=east, black] {};	
	
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X16) at (15, 7){};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X17) at (16, 7){};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X18) at (16, 8){};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X19) at (16, 6){};
	\draw[dashed, gray,  ->] (X16) -- (X19)  node[ anchor=east, black] {};
	\draw[dashed, gray,  ->] (X16) -- (X17)  node[ anchor=east, black] {};
	\draw[dashed, gray,  ->] (X16) -- (X18)  node[ anchor=east, black] {};	
	
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X20) at (14, 6){};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X21) at (15, 7){};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X22) at (15, 5){};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X23) at (15, 6){};
	\draw[dashed, gray,  ->] (X20) -- (X21)  node[ anchor=east, black] {};
	\draw[dashed, gray,  ->] (X20) -- (X22)  node[ anchor=east, black] {};
	\draw[dashed, gray,  ->] (X20) -- (X23)  node[ anchor=east, black] {};	
	
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X24) at (13, 5){};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X25) at (14, 4){};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X26) at (14, 5){};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X27) at (14, 6){};
	\draw[dashed, gray,  ->] (X24) -- (X25)  node[ anchor=east, black] {};
	\draw[dashed, gray,  ->] (X24) -- (X26)  node[ anchor=east, black] {};
	\draw[dashed, gray,  ->] (X24) -- (X27)  node[ anchor=east, black] {};	

	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X28) at (12, 5){};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X29) at (13, 6){};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X30) at (13, 5){};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X31) at (13, 4){};
	\draw[dashed, gray,  ->] (X28) -- (X29)  node[ anchor=east, black] {};
	\draw[dashed, gray,  ->] (X28) -- (X30)  node[ anchor=east, black] {};
	\draw[dashed, gray,  ->] (X28) -- (X31)  node[ anchor=east, black] {};	
	
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X32) at (11, 6){};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X33) at (12, 6){};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X34) at (12, 7){};
	\node[inner sep = \BallSize pt, ball color=\PayoffColor, circle] (X35) at (12, 5){};
	\draw[dashed, gray,  ->] (X32) -- (X33)  node[ anchor=east, black] {};
	\draw[dashed, gray,  ->] (X32) -- (X34)  node[ anchor=east, black] {};
	\draw[dashed, gray,  ->] (X32) -- (X35)  node[ anchor=east, black] {};		
	
	\node[xshift=-15] () at (2, 5) {{\LARGE$\mathsf{x}$}};	% 'x' label


        \foreach \t in {1, 2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 14, 15, 16, 17} { \node[ anchor=north, black] at ({\t+1}, 0) {$t_{\t}$}; }

